Adapting Pre-trained Language Models for Quantum Natural Language Processing

The emerging classical-quantum transfer learning paradigm has brought a decent performance to quantum computational models in many tasks, such as computer vision, by enabling a combination of quantum models and classical pre-trained neural networks. However, using quantum computing with pre-trained models has yet to be explored in natural language processing (NLP). Due to the high linearity constraints of the underlying quantum computing infrastructures, existing Quantum NLP models are limited in performance on real tasks. We fill this gap by pre-training a sentence state with complex-valued BERT-like architecture, and adapting it to the classical-quantum transfer learning scheme for sentence classification. On quantum simulation experiments, the pre-trained representation can bring 50\% to 60\% increases to the capacity of end-to-end quantum models.

==> src/backgrounds.tex <==
\section{Preliminaries}
\label{sec:tensor}

\subsection{Quantum Mechanics}
Quantum mechanics (QM), also known as quantum physics (QP) or quantum theory (QT), is a fundamental theory of physics that describes the world at a microscopic scale.  The behaviors of atomic and sub-atomic particles, such as electrons or photons, cannot be sufficiently explained by classical physics. Quantum mechanics has thus been gradually developed as both a conceptual and a mathematical framework to define the laws that the microscopic particles should obey.

The building blocks of the mathematical framework of quantum mechanics are the \textit{postulates}. The postulates of quantum mechanics vary slightly from place to place. This thesis follows the definitions of 4 postulates in Chapter 2 in~\cite{nielsen_quantum_2011}, because they are clearly stated and closely related to the thesis's theoretical framework. Next we introduce the postulates in a sequential manner, as well as the associated concepts relevant to this paper. Curious readers are referred to ~\cite{nielsen_quantum_2011} for a better understanding.

For better illustrations, we adopt the \textit{Dirac Notation} for a symbolic representation of quantum concepts. Essentially, a complex-valued \textit{unit} vector $\vec{\mu}$ and its conjugate transpose $\vec{\mu}^H$ (also denoted as $\vec{\mu}^\dagger$) are denoted as a \textit{ket} $\ket{u}$ and a \textit{bra} $\bra{u}$ respectively~\footnote{The conjugate of a complex number is the number with an equal real part and an imaginary part equal in magnitude, but opposite in sign}. The inner product of two unit vectors $\ket{u}$ and $\ket{v}$ is a \textit{braket} $\braket{u|v}$, and the complex-valued matrix representing their outer product is $\ket{u}\bra{v}$.

\subsubsection{States}~\label{chp:state}
\begin{postulate}
Associated with any isolated physical system is a complex vector space
with an inner product (that is, a Hilbert space) known as the \textbf{state space} of the system. The system is completely described by its \textbf{state vector}, which is a unit vector in the system's state space.
\end{postulate}

The first postulate talks about the space of any quantum system and the system's state on the space. Typically the Hilbert Space is denoted as $\mathcal{H}$, spanned by a set of mutually orthogonal bases $\{\ket{e_i}\}$, termed as \textit{basis states}.  The state of a single quantum system is described by a \textit{pure state} $\ket{\psi}$. For instance, an electron could be a single quantum system, and the state $\ket{\psi}$ describes its location or momentum. Mathematically, $\ket{\psi}$ could be written as a linear combination of basis states

\begin{equation}
    \ket{\psi} = w_1 \ket{e_1} + ...+ w_n \ket{e_n},
\end{equation}

where $\{w_j\}$ are complex scalars with $\sum_j |w_j|^2 = 1$, with $|\cdot|$ being the modulus of a complex number. The state of the system usually does not fall onto a basis state $\ket{e_j}$, but it is a superposition of the basis states, called a \textit{superposition state}. Superposition is one of the fundamental concepts in quantum mechanics that differs from classical physics. It means that a quantum system can be in different basis states simultaneously. For instance, the position of an electron can be anywhere, and the probability density function $\psi(x)$ of the electron at location $x$ in the space is a complex-valued scalar satisfying $\int |\psi(x)|^2 = 1$. Hence the position of an electron is a superposition state $\ket{\psi} = \sum \psi(x) \ket{x}$ on a infinite-dimensional Hilbert Space $~\mathcal{H^{\infty}}$ spanned by the basis states $\{\ket{x}\}$, each corresponding to a position $x$ in the space. The probability amplitude $\psi(x)$ is also called a \textit{wave function}. 
Another example is the simplest quantum mechanical system, called a \textit{qubit}, which is situated at a 2-dim Hilbert Space spanned by basis vectors $\ket{0}$ and $\ket{1}$. The general pure state of a qubit can be written as $\ket{\psi} = \alpha_0 \ket{0} + \alpha_1 \ket{1}$ with $|\alpha_0|^2 + |\alpha_1|^2 = 1$, corresponding to a point in the unit circle. Fig.~\ref{fig:state} below shows the states of the two examples above.

\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.98\linewidth]{Pics/bkg_superposition.png}
  \caption{Illustration of pure states. The left is the state of a qubit on a 2-dim Hilbert Space. The right is the probability density function for the location of an electron (in the 1-dimensional case), which is also a quantum state in the infinite-dimensional Hilbert Space.}
  \label{fig:state}

\end{figure}

\textit{Mixture} describes the overall state of a set of pure states on a common Hilbert Space $\mathcal{H}$. The statistical ensemble of such a mixed system of states is called a \textit{mixed state}, represented by a \textit{density matrix}. A density matrix $\rho$ is an Hermitian, positive semi-definite square matrix with unitary trace, i.e. $\rho =\rho^\dagger, \rho \geq 0, tr(\rho) = 1$. Essentially, for a set of pure states $\{\ket{\phi_j}\}_{j=1}^n$ with probability weights $\{p_j\}_{j=1}^n$, the density matrix $\rho$ of the mixed state is computed by
\begin{equation}   
\label{eq:mixture}
\rho = \sum_j^n p_j\ket{\psi_j}\bra{\psi_j}.
\end{equation}
Since $\{p_j\}_{j=1}^n$ are non-negative values that sum up to 1, the matrix $\rho$ produced by Eq.~\ref{eq:mixture} is always a legal density matrix. The diagonal elements of $\rho$ are always real non-negative values that sum up to 1, while the off--diagonal elements are general complex values. 

It is worth noting that mixture encodes the uncertainties in the distribution of particles. Different probabilistic weights of a set of pure states may yield identical (i.e. physically indistinguishable) mixed states. For instance, for the set of states $\{\ket{\psi_1} = [1,0], \ket{\psi_2} = [0,1], \ket{\psi_3} = [\frac{\sqrt 2}{2},-\frac{\sqrt 2}{2}], \ket{\psi_4} = [\frac{\sqrt 2}{2},\frac{\sqrt 2}{2}]\}$, we have $\frac{1}{2}\ket{\psi_1}\bra{\psi_1} + \frac{1}{2}\ket{\psi_2}\bra{\psi_2} = \frac{I_2}{2} = \frac{1}{2}\ket{\psi_3}\bra{\psi_3} + \frac{1}{2}\ket{\psi_4}\bra{\psi_4}$ ($I_2$ is the 2 by 2 identity matrix), so the distributions $\{\frac{1}{2},\frac{1}{2},0,0\}$ and $\{0,0,\frac{1}{2},\frac{1}{2}\}$ result in the same state.

Moreover, a pure state can be seen as a density matrix, i.e. $\rho = \ket{\psi_k}\bra{\psi_k}$ for some $k$. Hence the density matrix $\rho$ can be used to represent both a single quantum system (i.e. pure state) and a statistical ensemble of multiple systems (i.e. mixed state) in the same Hilbert space. 

A graphical illustration of a mixed state for a qubit is given in Fig.~\ref{fig:mixed_state}. Due to its probabilistic meaning, a mixed state is visually represented as an ellipsoid (i.e. an ellipse in the 2-dim case). In fact, it could be proved that, for a density matrix $\rho$, the plot of $\rho \ket{u}$ when a pure state $\ket{u}$ moves within the unit sphere is an ellipsoid, with the directions and lengths of axes being the eigenstates and eigenvalues of $\rho$ respectively. Hence the ellipsoid is a unique characterisation of the density matrix $\rho$.  

\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.5\linewidth]{Pics/bkg_mixture.png}
  \caption{Illustration of a mixed state in the 2-dim Hilbert Space. }
  \label{fig:mixed_state}
\end{figure}


\textit{Interference} is a key quantum phenomenon that cannot be explained from a classical point of view. It is a result of quantum superposition, in which different paths in superposition interfere with each other, bringing to an additional \textit{interference term} compared to the law of total probability in classical probability theory. 

The famous experiment that demonstrated the existence of interference was the \textit{Double Slit Experiment}. As is shown in Fig.~\ref{fig:double-slit-experiment}, a source of electrons was fired to a screen with two slits, namely $A$ and $B$. Another screen was set up behind the screen, with a detector that detected the distribution of particles arriving at the screen. From the distribution it was possible to calculate the probability of a particle at a particular position $x$ on the screen. First, the particle probability distribution was obtained when only A or B was open, shown in Fig.~\ref{fig:double-slit-experiment}a and Fig.~\ref{fig:double-slit-experiment}b respectively. Then, the distribution was calculated with both slits were open. Surprisingly, a fluctuating pattern (Fig.~\ref{fig:double-slit-experiment}c) was obtained instead of what was expected to be a linear combination of the respective distributions (Fig.~\ref{fig:double-slit-experiment}d). Put in a mathematical way, the probability distribution $p_{AB}(x)$ with both slits open was not a simple linear combination of the distributions $p_{A}(x)$ and $p_{B}(x)$, which violated the law of total probability.

\begin{figure}[ht!]
  \centering
  \includegraphics[width=\linewidth]{Pics/double_slit_experiment.png}
  \caption{Double-slit Experiment.}
  \label{fig:double-slit-experiment}
\end{figure}

The phenomena, however, could be well explained under the framework of quantum mechanics.  The electron was in state $\ket{\psi_A}$ and $\ket{\psi_B}$ respectively, when only one slit was open. According to Born's rule~\cite{born1926quantenmechanik}, the probability that the electron reaches a particular location $x$ was given by
\begin{eqnarray}
    p_{A}(x) &=& |\braket{\psi_A|x}|^2 \nonumber \\
    p_{B}(x) &=& |\braket{\psi_B|x}|^2.
\end{eqnarray}

When both slits are open, the electron passing the screen was however in a superposition of two-slit states, i.e. 

\begin{equation}
   \ket{\psi_{AB}} = \lambda_A \ket{\psi_A} + \lambda_B\ket{\psi_B}
\end{equation}

where $\lambda_A^2 + \lambda_B^2 = 1$ to ensure that $\ket{\psi_{AB}}$ is a physical state. The probability that the electron reached $x$ after passing both slits is then

\begin{eqnarray}
     p_{AB}(x) &=& |\braket{\psi_{AB}|x}|^2 \nonumber \\
    &=& |\lambda_A \braket{\psi_A|x} +\lambda_B \braket{\psi_B|x}|^2 \nonumber \\
    &=& \lambda_A^2 |\braket{\psi_A|x}|^2 +\lambda_B^2|\braket{\psi_B|x}|^2 + 2\lambda_A\lambda_B Re\{\braket{\psi_A|x}\braket{\psi_B|x}\} \nonumber \\
    &=& \lambda_A^2 p_A(x) +\lambda_B^2 p_B(x) +2\lambda_A\lambda_B p_A(x) p_B(x) cos(\phi_A(x)-\phi_B(x)),
\end{eqnarray}

where $\phi_A(x)$ and $\phi_B(x)$ are the phases of the complex values $\braket{\psi_A|x}$ and $\braket{\psi_B|x}$ respectively at position $x$. Compared to the classical law of total probability where $p_{AB}(x) = \lambda_A^2 p_A(x) +\lambda_B^2 p_B(x)$, an additional term $2\lambda_A\lambda_B p_A(x) p_B(x) cos(\phi_A(x)-\phi_B(x))$ appears. The phase difference $\phi_A(x)-\phi_B(x)$ is a function of position $x$ rather than a constant value, so the additional term has different values at different positions, with certain periodicity due to the cosine function. 

The additional term indicates the interference between the slits, and is hence called the \textit{interference term}. The appearance of this term is due to the superposition of the two slits when an electron passes. The superposition means the electron passes the screen via both slits simultaneously, while the classical probability theory suggests that the electron passes through either $A$ or $B$. 



\subsubsection{Evolution}

\begin{postulate}

The evolution of a closed quantum system is described by a \textbf{unitary transformation}. That is, the system state $\ket{\psi}$ at time $t_1$ is related to the state $\ket{\psi^\prime}$ at time $t_2$ by a unitary operator $U$ which depends only on the times $t_1$ and $t_2$, 
\begin{equation}
    \ket{\psi^\prime} = U\ket{\psi}
\end{equation}

\end{postulate}

The postulate speaks about the evolution of a quantum system over time. Although the definition requires a quantum system to be closed, an open system can be viewed as part of a larger closed system, so the concept of evolution universally applies.  The evolution is always manipulated by a unitary operator $U$, or equivalently a complex-valued unitary matrix on Hilbert Space $\mathcal{H}$. A unitary matrix is invertible and its inverse is identical to its Hermitian, i.e. $U^{-1} = U^\dagger$. 

The equation in the postulate mentions the evolution of a pure state. Since the unitary operator is inner product preserving, the result is also a pure physical state. For a system in mixed state $\rho = \sum_j^n p_j\ket{\psi_j}\bra{\psi_j}$, unitary evolution yields

\begin{eqnarray}
    \rho' &=& \sum_j^n p_j\ket{\psi_j'}\bra{\psi_j'} \nonumber \\
    &=& \sum_j^n p_j(U\ket{\psi_j}\bra{\psi_j}U^\dagger) \nonumber \\
    &=& U(\sum_j^n p_j\ket{\psi_j'}\bra{\psi_j'})U^\dagger \nonumber \\
    &=& U\rho U^\dagger,
\end{eqnarray}

\noindent hence $\rho' = U\rho U^\dagger$ describes the evolution of a general state in a single quantum system.

\noindent \textbf{Remark:} the postulate is derived from the solution of Schr{\"o}dinger's equation. In this paper, we use solely the unitary matrix $U$ for a formulation of evolution, so the introduction of Schr{\"o}dinger's equation and the mathematical derivation is omitted. Interested readers are referred to Chapter 2 of ~\cite{nielsen_quantum_2011} for details.

\subsubsection{Measurement}

\begin{postulate}
Quantum measurements are described by a collection ${M_m}$ of
\textbf{measurement operators}. These are operators acting on the state space of the system being measured. The index $m$ refers to the measurement outcomes that may occur in the experiment. If the state of the quantum system is $\ket{\psi}$ immediately before the measurement,  then the probability that result $m$ occurs is given by
\begin{equation}\label{eq:measurement_probability}
    p(m) = \bra{\psi} M_m^\dagger M_m \ket{\psi}
\end{equation}

and the state of the system after the measurement is 
\begin{equation}
    \frac{M_m \ket{\psi}}{\bra{\psi} M_m^\dagger M_m \ket{\psi}}.
\end{equation}

The measurement operators satisfy the completeness equation,
\begin{equation}\label{eq:completeness}
    \sum_m  M_m^\dagger M_m = I,
\end{equation} 

which means

\begin{equation}
    \sum_m p(m) = 1.
\end{equation} 

\end{postulate}

The postulate is concerned with the process of measuring a quantum physical system, such as the momentum of an electron. Prior to measurement, the system is in the uncertain state where it takes all the values $\{m\}$ simultaneously. The measurement allows the system to \textit{collapse} onto a single state, and only one of all possible values can be observed for each measurement. The probability that a particular value $m$ is observed is determined by the original system state and the operator $M_m$ corresponding to $m$. Since $\{m\}$ are all possible outcomes, the operators have to satisfy the completeness condition to guarantee the probabilities of all outcomes sum up to 1. 

The most common type of measurement is called \textit{projective measurement}. It is the case where the operators are projectors on a set of mutually orthogonal basis states, i.e. $M_m = \ket{m}\bra{m}$ with $\{\ket{m}\}$ spanning the Hilbert Space $\mathcal{H}$. In this way, the projective measurement is associated with an \textit{observable} $\hat{O}$, which is a square Hermitian matrix, i.e. $\hat{O} = \hat{O}^{\dagger}$\footnote{For simplicity, we chose a nomenclature instead of a strict definition. Please refer to~\cite{nielsen_quantum_2011} for a strict definition of projection measurement.}. It can be decomposed into 
\begin{equation} \label{eq:observable_spectrum_decomposition}
    \hat{O} = \sum_m m \ket{m}\bra{m},
\end{equation}
where $m$ and $\ket{m}$ are also called an \textit{eigenstate} and an \textit{eigenvalue} respectively. Suppose the system is in the state $\ket{\psi}$ prior to measurement. The calculation of probability $P(m)$ from Eq.~\ref{eq:measurement_probability} now becomes
\begin{eqnarray}\label{eq:born}
    p(m) &=& \bra{\psi} M_m^\dagger M_m \ket{\psi} \nonumber \\ 
        &=& \bra{\psi} (\ket{m}\bra{m}) \ket{\psi} \nonumber \\
        &=& |\braket{\psi|m}|^2.
\end{eqnarray}

After measurement the system collapses precisely onto the state $\ket{m}$. If the system is at a mixed state $\rho$ prior to measurement, then the trace rule is employed to compute the probability:
\begin{equation}\label{eq:born_2}
    p(m) = tr(\rho \ket{m}\bra{m}).
\end{equation}

This is called the Born's rule~\cite{born1926quantenmechanik}. It is a generalization of the Eq.~\ref{eq:born} with the latter corresponding to the case when $\rho = \ket{\psi}\bra{\psi}$. Whether the pre-measurement state is a pure or a mixed state, it will always collapse onto a particular eigenstate $\ket{m}$ at a probability of $p(m)$. Suppose the experiment can be repeated for infinite times, then the average outcome (i.e. expected value) of the measurement would be

\begin{eqnarray}\label{eq:expectation}
    E(\hat{O}) &=& \sum_m {mp(m)} \nonumber \\ 
        &=& \sum_m {mtr(\rho \ket{m}\bra{m})} \nonumber \\
        &=& tr(\rho \sum_m {m}\ket{m}\bra{m}) \nonumber \\
        &=& tr(\rho \hat{O}).
\end{eqnarray}

Also, the post-measurement state is a mixture of all measurement states $\ket{m}$ with measurement probability distribution, expressed as 

\begin{eqnarray}\label{eq:post-measurement-state}
    \hat{\rho} &=& \sum_m {\ket{m}\bra{m} p(m)} \nonumber \\ 
        &=& \sum_m {\ket{m} (\bra{m}\rho\ket{m})\bra{m}} \nonumber \\
        &=& \sum_m {(\ket{m}\bra{m})\rho(\ket{m}\bra{m})} \nonumber \\
        &=& \sum_m {M_m\rho M_m}.
\end{eqnarray}

We now move back to the general form of measurement mentioned in the postulate. Suppose we define $E_m = M_m^\dagger M_m$; then $E_m$ is a positive operator from elementary linear algebra. Since $\sum_m {E_m} = I$ (Eq.~\ref{eq:completeness}), the set of operators $\{E_m\}$ are called a  \textit{positive-operator valued measure (POVM)}, and each operator $E_m$ is a $POVM$ \textit{element}. The probability for value $m$ is given by $p(m) = tr(\rho E_m)$ for a system in state $\rho$ prior to measurement.

Let us consider the case of a 2-dimensional Hilbert Space spanned by $\ket{0}$ and $\ket{1}$. Suppose we have the two operators below:

\begin{eqnarray}
    E_+ &=& \frac{\eta}{2} I + (1-\eta)\ket{1}\bra{1} \nonumber \\
    E_- &=& \frac{\eta}{2} I + (1-\eta)\ket{0}\bra{0},
\end{eqnarray}

where $\eta \in [0,1]$. It is easy to check that $E_+$ and $E_-$ are both positive semi-definite density matrices (i.e. positive operators) satisfying $E_+ +E_- = I$, so $\{E_+,E_-\}$ is a $POVM$ set. However, for almost all values of $\eta \in [0,1]$, $E_+$ and $E_-$ are not mutually orthogonal, which means $\{E_+,E_-\}$ is not a projective measurement. In fact, it could be proved that $\{E_+,E_-\}$ is a projective measurement if and only if $\eta = 0$. When this happens, i.e., $\{E_+,E_-\} = \{\ket{1}\bra{1}, \ket{0}\bra{0}\}$, it means the measurement is taken along the basis states. The illustrates that \textit{POVM} is a generalization of projective measurements.

It is worth mentioning that the projective measurement is taken into consideration more often, even though \textit{POVM} is a more general form of measurement. The main reason is that a \textit{POVM} can be derived from a projective measurement: every \textit{POVM} is equivalent to a projective measurement on a larger Hilbert Space~\cite{nielsen_quantum_2011}. To some extent, it is sufficient to consider projective measurements for the description of quantum systems.


\subsubsection{Composite Systems}

\begin{postulate}

The state space of a composite physical system is the tensor product
of the state spaces of the component physical systems. Moreover, if we have
systems numbered $1$ through $n$, and system number $i$ is prepared in the state
$\ket{\psi_i}$, then the joint state of the total system is $\ket{\psi_1} \otimes \ket{\psi_2} \otimes ... \otimes \ket{\psi_n}$.
\end{postulate}

The fourth and last postulate is concerned with the \textit{composite quantum system} composed of two or more individual quantum systems. Suppose we have $n$ systems in composition, each located at Hilbert Spaces $\mathcal{H}_1,...,\mathcal{H}_n$ respectively. The composite system space $\mathcal{H}$ is then a tensor product of the Hilbert Spaces, i.e. $\mathcal{H} = \mathcal{H}_1 \otimes \mathcal{H}_2 \otimes ... \otimes \mathcal{H}_n$. Essentially, for any combination of basis states $\ket{e_{k_j}} \in \mathcal{H}_j, j = 1,...,n$, their tensor product $\ket{e_k} = \ket{e_{k_1}} \otimes  \ket{e_{k_2}} \otimes  ... \otimes \ket{e_{k_n}}$ is a basis state on $\mathcal{H}$.\footnote{The tensor product of two matrices $A = [A_{ij}]$ and $B = [B_{kl}]$ is $A \otimes B = [A_{ij}B]$. A pure state is a row vector or a column vector and hence can be seen as a 1-by-$n$ or an $n$-by-1 matrix} Consequently, the dimension of the composite system is the multiplication of the dimensions of its component systems. In the same way as the single quantum system, pure states, superposition states and mixed states are properly defined on the composite system $\mathcal{H}$.

A crucial concept unique to composite quantum systems is \textit{entanglement}. Entanglement describes the state of a system which consists of more than one particle (e.g. photons) twisted together in such a way that the measurement outcome on a particle has an impact on the outcomes of other particles. For example, the polarization of two photons can be entangled, so that the polarization of one photon changes the polarization of the other, even though they are a large distance away from each other.

Mathematically speaking, entanglement means that the state of a many-particle system is not separable, i.e. cannot be factored as a product of states of constituent particles. Suppose, for simplicity, we have a system composed of two particles $A,B$, and located at $\mathcal{H}_{AB} = \mathcal{H}_A \otimes \mathcal{H}_B$.  A pure state $\ket{\psi} \in \mathcal{H}_{AB}$ is \textit{separable} if and only if there exists $\ket{\psi^A} \in \mathcal{H}_A$ and $\ket{\psi^B} \in \mathcal{H}_B$ such that  
\begin{equation}
    \ket{\psi} = \ket{\psi^A} \otimes \ket{\psi^B},
\end{equation}
otherwise $\ket{\psi}$ is called an \textit{entangled pure state}. The concept of entanglement also holds for mixed states but is slightly different from the pure state case. A mixed state $\rho \in \mathcal{H}_{AB}$ is separable if and only if it can be written as

\begin{equation}
    \rho = \sum_j w_j \rho_j^A \otimes \rho_i^B,
\end{equation}

\noindent where $w_j \in \mathcal{R}$, $\rho_j^A \in \mathcal{H}_A$ and $\rho_j^B \in \mathcal{H}_B$ for any $j$. When $\rho$ cannot be decomposed as above, it is entangled and hence called an \textit{entangled mixed state}.

Entanglement induces a profound difference between quantum correlation, which is computed for one single system, and classical correlation, which is computed for an ensemble. Consider one system in superposed state and one variable.  In QM, the uncertainty of the measurement of the variable is derived from the superposition. If the superposed system consists of two subsystems tensored together, the correlation between the observation of the variable in one subsystem and the observation of the variable in the other subsystem is caused by the fact that the two systems are combined into one single system.  When entanglement exists, the (quantum) correlation can violate some statistical inequalities that cannot be violated when classical correlation is computed.

\textit{Reduced Density Matrix} is utilized to construct representations of sub-systems from a composite quantum system. Suppose we have a state $\rho \in \mathcal{H}_{AB}$ for a bi-particle system composed of systems $A$ and $B$. We would like to know the statistical equivalence of $\rho$ on only one system $A$, i.e. $\rho^A$. In other words, we are interested in finding the density matrix $\rho^A$ of system $A$ so that applying any measurement $M \in \mathcal{H}_A$ onto it yields the same result as applying the measurement $M \otimes I$ on the composite system state $\rho$ with system $B$ unchanged. According to Born's rule, we have

\begin{equation}
    tr(M \rho^A ) = tr( (M \otimes I_B)\rho), \forall M \in \mathcal{H}_A
\end{equation}

The reduced density matrix $\rho^A$ that satisfies this equation can be obtained by taking the \textit{partial trace} of $\rho$ over system $B$:

\begin{equation}
   \rho^A = tr_B(\rho),
\end{equation}

\noindent where the partial trace is defined as follows: suppose $\rho$ is represented as a linear combination of basis states
\begin{equation}
    \rho = \sum_{ijkl} c_{ijkl} \ket{e_i}_A\bra{e_j} \otimes \ket{f_k}_B\bra{f_l},
\end{equation}

where $\{\ket{e_i}\}$ and $\{\ket{f_j}\}$ span $\mathcal{H}_A$ and $\mathcal{H}_B$ respectively; then 
\begin{equation}
    \rho_A = tr_B(\rho) =  \sum_{ijkl} c_{ijkl} \braket{f_l|f_k}\ket{e_i}\bra{e_j}
\end{equation}
In the matrix form, taking partial trace is done by computing traces for all blocks corresponding to each subsystem partition. Fig.~\ref{fig:partial_trace} shows the case of taking the partial trace over a 2-qubit system state.  The partial trace operation obeys commutative law, so the reduced density matrix can be properly defined over any subset of the system of arbitrary scale (i.e. number of particles). 

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.8\linewidth]{Pics/partial_trace.png}
  \caption{Illustration of partial trace. The left-hand side is a density matrix of a two-qubit system. The partial trace is performed over system $B$. The right hand side shows the resulting 2 by 2 reduced density matrix of system $A$.}
  \label{fig:partial_trace}
\end{figure}


The reduced density matrix is indispensable in the analysis of composite quantum systems~\cite{nielsen_quantum_2011}. It has a wide range of applications in quantum information and communication, such as \textit{quantum teleportation}. 


\subsection{Quantum Probability} 

Quantum probability (QP) is a generalization of the classical probability theory. It sets up the mathematical foundations of quantum mechanics and provides a probabilistic interpretation of quantum mechanics concepts. By using such terminologies as events and measures, a probabilistic view on the quantum states and measurements is given.

There are five key concepts vital to any probability theory: measurable space, probability measure, random variable, probability distribution and expectation value~\cite{kolmogorov_foundations_1950}. The difference between quantum probability and the classical probability is rooted in the measurable spaces on which the probability measure is defined.  In particular, the classical probability is defined on subsets of a set of elements subject to union and intersection operations. Likewise, the quantum probability is defined on subspaces of a Hilbert Space with properly defined meet and join operations. However, the two structures are different in that the former submits to the distributive law while the latter does not necessarily submits to this law. In mathematical language, \textit{the former is isomorphic to a binary lattice while the latter is isomorphic to a general lattice}~\cite{jauch_structure_1975}.  

This means that quantum probability is a generalization of classical probability with the removal of the distributive law. The difference is actually a reflection of a crucial concept in quantum mechanics: it could be proved that the distributive law in the operations of subspaces on a Hilbert Space is equivalent to the commutative law of projections on subspaces~\cite{jauch_structure_1975}. In this way, quantum probability can be seen as a non-commutative analog of classical theory.

The bridge between the mathematical theory of quantum probability and the physical formalism of quantum mechanics is \textit{Gleason's Theorem}~\cite{gleason1957measures}. Gleason's Theorem proves that a probability measure on the Hilbert Space is uniquely represented by a density operator (i.e., density matrix), and the approach to compute probabilities on a Hilbert Space is in a similar form as in Born's rule. Based on Gleason's Theorem, the states and measurements in quantum mechanics could be naturally derived. 

\subsubsection{Events}
In quantum probability, \textit{events} are defined as subspaces or, equivalently, projectors on subspaces. A projector is mathematically a square matrix $P$ such that $P^2 = P$. In particular, an \textit{elementary element} is a 1-dimensional subspace, represented as $\ket{u}\bra{u}$, also called a \textit{dyad}.

\subsubsection{Measures}

According to the axiomatic definition of probability theory~\cite{kolmogorov_foundations_1950}, a quantum probability measure $\mu(\cdot)$ is defined on the Hilbert Space such that 

(i) $\mu(\ket{u}\bra{u}) \in [0,1]$ for every elementary event $\ket{u}\bra{u}$
(ii) $\sum_j \mu(\ket{u_j}\bra{u_j}) = 1$ for any set of elementary events $\{\ket{u_j}\}$ that form an orthonormal basis.

Gleason's Theorem states that, for a Hilbert Space with a dimension greater than 2, there exists a one-to-one correspondence between a quantum probability measure $\mu(\cdot)$ and a density matrix $\rho$, and the value of quantum probability for any event $P$ is given by

\begin{equation}\label{eq:gleason}
    \mu_{\rho} (P) = tr(\rho P).
\end{equation}

In particular, the probability of an elementary event is 
\begin{equation}\label{eq:gleason_ele}
    \mu_{\rho} (\ket{u}\bra{u}) = tr(\rho \ket{u}\bra{u}) = \bra{u}\rho\ket{u}
\end{equation}

To this point, we are able to map the concepts in quantum mechanics to QP notions. The state of a single quantum system is a density matrix $\rho$, which determines a probability measure on the space. Operators of a projective measurement are events where an operator is an elementary event $\ket{u}\bra{u}$ most of the time. In cases where a value corresponds to multiple mutually orthogonal operators, it also corresponds to a projector on a high-dimensional subspace spanned by the orthogonal operators. In this way, Born's rule in Eq.~\ref{eq:born_2} that computes the measurement probability is identical to Gleason's Theorem in Eq.~\ref{eq:gleason}.  

The evolution of states and states of composite systems also adopt a quantum probability interpretation. However, they are omitted since they are not used either in this thesis or any related work. Interested readers are referred to~\cite{redei_quantum_2007} for a detailed look.

\subsubsection{Entropy}

In the information theory, an entropy could be defined for a probability distribution. Since a density matrix $\rho$ determines a quantum probability distribution on the Hilbert Space, its quantum entropy could be similarly defined as
\begin{eqnarray}\label{eq:entropy}
    S(\rho) &=& -tr(\rho log \rho) \nonumber \\
            &=& -\sum_j \lambda_j log \lambda_j \\,
\end{eqnarray}

where $\{\lambda_j\}$ are the set of eigenstates of $\rho$. The density matrix  
entropy is also called \textit{Von Neumann Entropy}, which determines the quantum information contained in the density matrix.


% % The uncertainty is one of the key foundations in the QT. The \emph{superposition} implies the uncertainty for a single particle while uncertainty for an ensemble system with multiple particles is described in a mixed system with measurement operations.

% \subsubsection{Superposition}
%  Algebraically, a particle in microscope world (e.g. atoms or photons) is described by vectors a multi-dimensional space. In a 2-dimensional case, in which two basis vectors are named as $\ket{0}$ and $\ket{1}$, \emph{Superposition} can be implemented as a linear combination of the basis vectors with complex-valued weights.  
% \begin{equation}   
% \ket{\phi} = \alpha_0 \ket{0} + \alpha_1 \ket{1}, 
% \end{equation} 
% where $0 \leq |\alpha_0|^2 \leq 1 $, $0 \leq |\alpha_1|^2 \leq 1 $  and $ |\alpha_0|^2 + |\alpha_1|^2 = 1$.  $\alpha$'s are complex scalars and $\ket{0}$ and $\ket{1}$ are vectors in complex vector space.   
% %The state $\ket{\phi}$ is said to be a superposition of the states $\ket{0}$ and $\ket{1}$, and the scalars $\alpha_0$ and $\alpha_1$ denote the amplitudes of the superposition. 
% %When either $|\alpha_0|^2$ or $|\alpha_1|^2$ is $1$, the particle corresponds to a classical bit; when $|\alpha_0|^2 = 1$, then $|\alpha_1|^2 = 0$ and $\ket{\phi} = \ket{0}$, and vice versa. It can be shown that the general particle state vector is normalized. 

% \subsubsection{Mixed system and Measurements}
% An ensemble system with multiple particles is called a \emph{mixed system}, in which the probability distribution is encapsulated by  a  positive semi-definite with unitary trace i.e. density matrix  
% \begin{equation} 
% \rho = \alpha_i \ket{\phi_i} \bra{\phi_i} 
% \end{equation} 
% In order to infer the possible state of this mixed system, Gleason's theorem \cite{gleason1957measures,hughes1992structure} is used  to calculate probability in quantum physics through measurements $\ket{M}$, i.e.
% \begin{equation} 
% \label{trace_measurement}
% P_M(\rho) =  \bra{M} \rho \ket{M} =tr(\rho \ket{M} \bra{M} ) 
% \end{equation}
% Although the off-diagonal elements pf $\rho$ is complex-valued, the $P_M(\rho)$  is guaranteed to be real-valued, since both  $\rho$ and $\ket{M} \bra{M}$ are Hermitian.

% \subsection{Semantic Hilbert Space}
% \label{semantic_hilbert_space}
% Here we introduce the Semantic Hilbert Space $\mathcal{H}$ defined on a complex vector space $\mathcal{C}^n$, and three different linguistic units, namely sememes, words and word combinations on the space. The concept of semantic measurement is introduced at last.

% % For convenience purposes, we follow the Dirac notations, which are widely used in quantum probability. Basically, a unit vector $\vec{\mu}$ and its transpose $\vec{\mu}^T$ are denoted as a ket $\vert u \rangle$ and a bra $\langle u \vert$ respectively. 

% % \subsubsection{Sememe}

% \textbf{Sememes.} 
% We assume $\mathcal{H}$ is spanned by the set of orthogonal basis states $\{\ket{e_j}\}_{i=1}^n$ for \textit{sememes}, which are the minimum semantic units of word meanings in language universals~\cite{goddard1994semantic}. Semantic units with larger granularities are based on the set of sememe basis.

% % \subsubsection{Word}
% % \label{sec:word}
% \textbf{Words.} 
% Words are  composed of sememes in superposition. Each word $w$ is a superposition over all sememes $\{\ket{e_j}\}_{i=1}^n$, or equivalently a unit-length vector on $\mathcal{H}$:
% \begin{equation}
% \label{superposition}
% \vert w \rangle =  \sum_{j=1}^n r_j e^{i\phi_j} \vert e_j \rangle
% \end{equation}
% In the expression above, $\{r_j\}_{j=1}^n$ are non-negative real-valued amplitudes satisfying $\sum_{j=1}^n {r_j}^2$ =1 and $\phi_j \in [-\pi,\pi]$ are the corresponding complex phases. 

% % We could also transfer the complex number in a complex plane as $re^{i\phi} = \cos\phi + i\sin\phi $.

% % We assume there are $n$ semantic concepts $\{C_i\}_{i=1}^{n}$ in the text collection, which could be considered as a limited The Hilbert Space $\mathcal{H}$ is then an n-dimensional finite space, where the concepts form a set of pure orthonormal states of the space, denoted as $\{\vert e_i \rangle\}_{i=1}^n$. 

% % \subsubsection{Semantic Composition}
% % \label{sentence_rep}
% \textbf{Semantic Composition.} 
% We view a combination of words (e.g. phrase, $n$-gram, sentence or document) as a mixed system composed of individual words, and its representation is computed as follows:
% \begin{equation}
% \label{mixture_old}
% \rho = \sum^m_j { \frac{1}{m} \ket{w_j} \bra{w_j}},
% \end{equation}
% where $m$ is the number of words and $\ket{w_j}$ is word superposition state in Eq.~\ref{superposition}, allowing multiple occurrences. Eq.~\label{mixture_old} produces a density matrix $\rho$ for semantic composition between words.
% %It describes a non-classical distribution over the set of sememes:  the complex-valued off--diagonal elements describes the correlations between sememes, while the diagonal entries (guaranteed to be real by its original property) correspond to a standard probability distribution. The off--diagonal elements provide our framework some potentials to model the possible interactions between the basic sememe basis, which was usually considered mutually independent with each other.

% %, which may give rise to emerging meanings when words are combined. 

% % \subsubsection{Semantic Measurement}
% \textbf{Semantic Measurement.} 
% The high-level features of a sequence of words are extracted through
% measurements on its mixed state. Given a density matrix $\rho$ of a mixed state, a rank-one projector $P$, which is the outer product of a unit complex vector, i.e. $P_{M_i}=\ket{M_i}\bra{M_i}$, is applied as a measurement projector. It is worth mentioning that $\ket{M_i}$ could be any state in this Hilbert space (not only limited to a specific word $w$).
% The measured probability is computed by Gleason`s Theorem ( Eq.~\ref{trace_measurement}), namely $P_{M_i}(\rho) =  \bra{M_i} \rho \ket{M_i} =tr(\rho \ket{M_i} \bra{M_i}$  . The measurement directions i.e. $\{\ket{M_i}\}_{i=0}^{n}$ are mutually orthogonal with each other, therefore we can get a normalized  multinomial probability distribution $\sum_{i=0}^{n}(P_{M_i}(\rho)) =1$.





% The advantages of the above Semantic Hilbert Space are threefold. First,  similarly to capsules \cite{sabour2017dynamic} and quaternions RNN \cite{parcollet2018quaternion}, Semantic Hilbert Space (SHS) can code internal dependencies by composing and processing multidimensional
% features as single entities, namely unitary states.
% Second, the measurements can be treated as general feature extractor based on some general pre-trained language model \cite{devlin2018bert}, which can provide some potential to transfer the learned measurements from a dataset to a new dataset. Finally, the words and measurements are embedded in a single Hilbert Space, making this framework easy to be understood by humans. Thus the model can be more robust and possible to be managed by manual adjustment.


\subsection{Tensors and the Tensor Product}

A \emph{tensor} is a natural way to describe certain objects that have a central role in modern quantum physics and beyond.  
% Compared to matrices and vectors, tensor is not very common-used in machine learning communities. However, tensors are everywhere and  it is getting more and more attentions.
A tensor is, roughly, a multi-dimensional array with certain composition properties. For example, A first-order tensor over the space
$\mathbb{R}^m$ is a vector ${\bf{v}} \in \mathbb{R}^{m}$ \footnote{In the rest of this paper, we also regard a matrix as a kind of tensor, namely  a 2-order tensor.}, and a second-order tensor is a matrix.  There are typical ways to build tensors through a set of matrices or vectors, namely \textit{stacking} and \textit{tensor product}.

\textbf{Stacking.} 
Stacking a series of $n$-order tensors could result in $n+1$-order tensors, namely, let $\tG_{1},\tG_{2} \cdots,\tG _{r_{n+1}} \in \mathbb{R}^{r_1 r_2 \cdots r_n}$,
\begin{equation}
[\tG_{1};\tG_{2} \cdots;\tG _{r_{n+1}} ] \in \mathbb{R}^{r_1 r_2 \cdots r_n r_{n+1}}
\end{equation}
In detail, the typical basic feature arrays  are  pixels of images in computer vision and  words of textual documents in natural language processing. It is commonly-used to stack the pixels with vertical and horizontal directions, resulting $\textrm{width} \times \textrm{height}$ 2-order matrices. Similarly, words, which are usually represented as distributed vectors, can be stacked as matrices while they are sequentially occurring in a document.
High-order arrays i.e. tensors are usually built by stacking with more than 2 dimensions. The extra orders \footnote{It is worthy mentioned that  data/features in a \textit{batch} can be stacked in deep learning approaches, resulting in a new order related to \textit{batch}; therefore, this is one of the reasons why Google named its deep learning framework as Tensorflow, that is a \textit{data flow with tensors}.} can be 1) \textbf{timestamp}: data which involves time, like google books and Arxiv paper collections; 2)  \textbf{modality}: data with multiple modality e.g. image, text and sound; 3) \textbf{domain}: data with multiple domains, like news in sport, economy and politics. 4)  \textbf{positional order}: data with a sequential order, for example, language;




\textbf{Tensor Product.} 
%The \textbf{order} of a tensor is defined to the number of indexing entries in the array, which are referred to as modes. The dimension of a tensor in particular mode is defined as the number of values that may be taken by the index in the mode. 
%A tensor $\mathcal{T} \in \mathbb{R}^{m_1 \times \ldots \times m_n}$ means that it is a $n$-order tensor with $m_i$ in each mode. 
\textit{Tensor product}, denoted by $ \otimes $, is typically as an operation on (pairs of) ordered set of objects, for example, sequential data like zig-zag pixels in images and tokens/words in text. Let $\tA \in \mathbb{R}^{m_{1}\times\cdots\times m_{I}}$ and $\tB \in \mathbb{R}^{m_{I+1}\times\cdots\times m_{J}}$ be tensors of orders $I$ and $J$, respectively. Then, $\tA \otimes \tB \in \mathbb{R}^{m_{1}\times\cdots\times m_{I+J}}$ is a tensor of order ${I+J}$.
The dimension of the tensor product between two tensors is  the product of the dimensions thereof, which is especially for sequential data like zig-zag pixels in images and tokens/words in text. 
The below is the example of the tensor product between two 2-order tensors (namely matrices):
\begin{equation}
\begin{aligned}
\begin{bmatrix}
 a_{1,1} & a_{1,2} \\
 a_{2,1} & a_{2,2} \\
 \end{bmatrix}
\otimes
 \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix}
&=
 \begin{bmatrix}
 a_{1,1} \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix} & a_{1,2} \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix} \\
 & \\
 a_{2,1} \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix} & a_{2,2} \begin{bmatrix}
 b_{1,1} & b_{1,2} \\
 b_{2,1} & b_{2,2} \\
 \end{bmatrix} \\
 \end{bmatrix} \\
&=
 \begin{bmatrix}
  \begin{bmatrix}
 a_{1,1} b_{1,1} & a_{1,1} b_{1,2} & \\ a_{1,2} b_{1,1} & a_{1,2} b_{1,2} \\
  \end{bmatrix}
  \begin{bmatrix}
 a_{1,1} b_{2,1} & a_{1,1} b_{2,2} & \\ a_{1,2} b_{2,1} & a_{1,2} b_{2,2} \\
  \end{bmatrix} \\
  \begin{bmatrix}
 a_{2,1} b_{1,1} & a_{2,1} b_{1,2} & \\ a_{2,2} b_{1,1} & a_{2,2} b_{1,2} \\
  \end{bmatrix}
  \begin{bmatrix}
 a_{2,1} b_{2,1} & a_{2,1} b_{2,2} & \\ a_{2,2} b_{2,1} & a_{2,2} b_{2,2} \\
 \end{bmatrix}
 \end{bmatrix}.
\end{aligned}
\end{equation}
%We use
%<\cdot, \cdot>$ for the inner product between two tensors in same space, i.e., the sum of element-wise multiplication of two tensors.
% $\mathbb{R}^{m_{1}\times\cdots\times m_{I}}$
Let $\tT_{h_1,\cdots,h_n}  \in \mathbb{R}$ be a specific entry in a tensor. 
%$\tT$ will be referenced with subscripts, e.g. $\{h_1,\cdots,h_n\}$. 
The inner product of two same-sized tensors in $\mathbb{R}^{m_{1}\times\cdots\times m_{I}}$ is defined as 
\begin{equation}
    <\tA, \tB> = \sum_{ \{h^{(1)}, h^{(2)}, \cdots h^{(n)}\} \in \mathbb{I}} \mathcal{\tA}_{h_1,\cdots,h_n} \mathcal{\tB}_{h_1,\cdots,h_n}
\end{equation}
where $\mathbb{I}$ is the index set of with dimension ${m_{1}\times\cdots\times m_{I}}$.

% A special $n$-order tensor $\delta \in \mathbb{R}^{k \times\ldots \times k }$, is as follows~\cite{2017arXiv170401552L,2015arXiv150905009C}:
% \begin{equation}
% \label{eq:function}
% {\delta _{{h_1}\ldots{h_n}}} = \left\{ \begin{array}{l}
% 1,\begin{array}{*{20}{c}}
% {}&{{h_1} = \dots = {h_n}}
% \end{array}\\
% 0,\begin{array}{*{20}{c}}
% {}&{otherwise}
% \end{array}
% \end{array} \right.
% \end{equation}
% with ${h_i} \in \left[ k \right]$. It means that it's $1$ for diagonal elements, $0$ for non-diagonal elements. It is mainly to construct the decomposition equivalent to Tensor Network (TN).


\subsection{Tensor  Decomposition}
\label{sec:ttd}

In practical applications, tensors usually involve operations on high-dimensional spaces, whence tensor decomposition is adopted to reduce the computing time. CP (CANDECOMP/Parafac) Decomposition and Tucker Decomposition (also called Multilinear SVD or M-mode SVD) are most typical ways.
CP decomposition fits the given tensor with a linear combination of some rank-1 tensors, whereas Tucker decomposition computes the orthonormal mode matrices of the tensor. However, the expressive power of  CP decomposition  is limited due to that it is a sum of only some rank-one tensors, and Tucker Decomposition has exponential in d number of parameters i.e., $\mathcal{O}(dnr+r^d)$, leading it to be only widely used for relatively-lower dimension especially three-dimensional tensor~ \cite{oseledets2011tensor}. 

For high-order tensors, Tensor Train Decomposition~ \cite{oseledets2011tensor} 
is an alternative way to approximate a high-order tensor with a collection of 3-order tensors~\footnote{The first and last tensors have order 2, but we can generally treat them as 3-order tensors with a extra dummy order of length one. }, which increases only linearly to the dimension (order) of the tensor.

For a given tensor $\tA \in \mathbb{R}^{m_1\times m_2 \times \cdots \times m_n}$, one wishes to find tensors $\mG_1, \tG_2, \ldots,\tG_{n-1} , \mG_n$ such that:
\begin{equation}
\begin{aligned}
&\mG_1 \in \mathbb{R}^{m_1 \times r_1} \\
&\tG_2 \in \mathbb{R}^{r_1 \times m_2 \times r_2}\\
&\vdots \\
&\tG_i \in \mathbb{R}^{r_{i-1} \times m_i \times r_i}\\
&\vdots \\
&\mG_n \in \mathbb{R}^{r_{n-1} \times m_n }
\end{aligned}
\end{equation}
such that
\begin{equation}
\label{eq:ttdecomposition}
\tA = \mG_1  \tG_2  ... \tG_{n-1}  \mG_n \in \mathbb{R}^{m_1\times m_2 \times \cdots \times m_n}
\end{equation}


where $*$ is the matrix multiplication operation and will be omitted in the following part of this paper. Observe that Eq.~\ref{eq:ttdecomposition} only involves the multiplications of 3-order tensors, resulting in efficient space and time cost \cite{oseledets2011tensor}. 





==> src/checklist.tex <==
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> src/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

